Reverse image filtering using total derivative approximation and accelerated gradient descent

In this paper, we address a new problem of reversing the effect of an image filter, which can be linear or nonlinear. The assumption is that the algorithm of the filter is unknown and the filter is available as a black box. We formulate this inverse problem as minimizing a local patch-based cost function and use total derivative to approximate the gradient which is used in gradient descent to solve the problem. We analyze factors affecting the convergence and quality of the output in the Fourier domain. We also study the application of accelerated gradient descent algorithms in three gradient-free reverse filters, including the one proposed in this paper. We present results from extensive experiments to evaluate the complexity and effectiveness of the proposed algorithm. Results demonstrate that the proposed algorithm outperforms the state-of-the-art in that (1) it is at the same level of complexity as that of the fastest reverse filter, but it can reverse a larger number of filters, and (2) it can reverse the same list of filters as that of the very complex reverse filter, but its complexity is much smaller.

==> AGD_Results.tex <==

\begin{figure*}[h!]
\centering     %%% not \center


\begin{subfigure}{0.3 \textwidth}
 \caption{Gaussian Filter}
\begin{tikzpicture}
\tikzstyle{every node}=[font=\small]
\begin{axis}[
	x tick label style={/pgf/number format/1000 sep=},
	height=5cm,
    width=\textwidth,
	ylabel=PSNR,
	enlargelimits=0.1,
	legend style={at={(0.5,1.1)},
	anchor=center,legend columns=-1},
	ybar,
	bar width = .1 cm,
	%ybar interval=0.7,
	symbolic x coords={GD,MGD,NAG,RMSprop,ADAM,Adadelta}, % these are the specification of coordinates on the x-axis. 
	xtick={GD,MGD,NAG,RMSprop,ADAM,Adadelta},  
x tick label style={rotate=45,anchor=east, font=\small}
]
\addplot 
	coordinates {(GD,38) (MGD,46)(NAG,47) (RMSprop,37) (ADAM,39) (Adadelta, 38)};
\addplot 
	coordinates {(GD,31) (MGD,34)(NAG,34) (RMSprop,31) (ADAM,29)(Adadelta,34)};
\addplot 
	coordinates {(GD,31) (MGD,33)(NAG,33) (RMSprop,31) (ADAM,29)(Adadelta,32)};
%\legend{T,P,TDA}
\end{axis}
\end{tikzpicture}
   
\end{subfigure}
\begin{subfigure}{0.3 \textwidth}
 \caption{AMF}
\begin{tikzpicture}
\tikzstyle{every node}=[font=\small]
\begin{axis}[
	x tick label style={/pgf/number format/1000 sep=},
	height=5cm,
    width=\textwidth,
	ylabel=PSNR,
	enlargelimits=0.1,
	legend style={at={(0.5,1.1)},
	anchor=center,legend columns=-1},
	ybar,
	bar width = .1 cm,
	%ybar interval=0.7,
	symbolic x coords={GD,MGD,NAG,RMSprop,ADAM,Adadelta}, % these are the specification of coordinates on the x-axis. 
	xtick={GD,MGD,NAG,RMSprop,ADAM,Adadelta},  
x tick label style={rotate=45,anchor=east, font=\small}
]
\addplot 
	coordinates {(GD,44) (MGD,40)(NAG,42) (RMSprop,41) (ADAM,39) (Adadelta, 44)};
\addplot 
	coordinates {(GD,34) (MGD,33)(NAG,28) (RMSprop,31) (ADAM,34)(Adadelta,33)};
\addplot 
	coordinates {(GD,29) (MGD,34)(NAG,35) (RMSprop,31) (ADAM,33)(Adadelta,34)};
%\legend{T,P,TDA}
\end{axis}
\end{tikzpicture}
   
\end{subfigure}
\begin{subfigure}{0.28 \textwidth}
 \caption{AnisGF}
\begin{tikzpicture}
\tikzstyle{every node}=[font=\small]
\begin{axis}[
	x tick label style={/pgf/number format/1000 sep=},
	height=5cm,
    width=\textwidth,
	ylabel=PSNR,
	enlargelimits=0.1,
	legend style={at={(0.5,1.1)},
	anchor=center,legend columns=-1},
	ybar,
	bar width = .1 cm,
	%ybar interval=0.7,
	symbolic x coords={GD,MGD,NAG,RMSprop,ADAM,Adadelta}, % these are the specification of coordinates on the x-axis. 
	xtick={GD,MGD,NAG,RMSprop,ADAM,Adadelta},  
x tick label style={rotate=45,anchor=east, font=\small}
]
\addplot 
	coordinates {(GD,32) (MGD,32)(NAG,20) (RMSprop,23) (ADAM,28) (Adadelta,20 )};
\addplot 
	coordinates {(GD,23) (MGD,23)(NAG,11) (RMSprop,19) (ADAM,25)(Adadelta,17)};
\addplot 
	coordinates {(GD,24) (MGD,24)(NAG,14) (RMSprop,19) (ADAM,25)(Adadelta,16)};
%\legend{T,P,TDA}
\end{axis}
\end{tikzpicture}
   
\end{subfigure}
\begin{subfigure}{0.28 \textwidth}
 \caption{BF}
\begin{tikzpicture}
\tikzstyle{every node}=[font=\small]
\begin{axis}[
	x tick label style={/pgf/number format/1000 sep=},
	height=5cm,
    width=\textwidth,
	ylabel=PSNR,
	enlargelimits=0.1,
	legend style={at={(0.5,1.1)},
	anchor=center,legend columns=-1},
	ybar,
	bar width = .1 cm,
	%ybar interval=0.7,
	symbolic x coords={GD,MGD,NAG,RMSprop,ADAM,Adadelta}, % these are the specification of coordinates on the x-axis. 
	xtick={GD,MGD,NAG,RMSprop,ADAM,Adadelta},  
x tick label style={rotate=45,anchor=east, font=\small}
]
\addplot 
	coordinates {(GD,46) (MGD,35)(NAG,35) (RMSprop,40) (ADAM,39) (Adadelta, 46)};
\addplot 
	coordinates {(GD,34) (MGD,38)(NAG,37) (RMSprop,34) (ADAM,35)(Adadelta,40)};
\addplot 
	coordinates {(GD,34) (MGD,39)(NAG,32) (RMSprop,34) (ADAM,35)(Adadelta,38)};
%\legend{T,P,TDA}
\end{axis}
\end{tikzpicture}
   \end{subfigure}
\begin{subfigure}{0.28 \textwidth}
 \caption{RF}
\begin{tikzpicture}
\tikzstyle{every node}=[font=\small]
\begin{axis}[
	x tick label style={/pgf/number format/1000 sep=},
	height=5cm,
    width=\textwidth,
	ylabel=PSNR,
	enlargelimits=0.1,
	legend style={at={(0.5,-0.6)},
	anchor=center,legend columns=-1},
	ybar,
	bar width = .1 cm,
	%ybar interval=0.7,
	symbolic x coords={GD,MGD,NAG,RMSprop,ADAM,Adadelta}, % these are the specification of coordinates on the x-axis. 
	xtick={GD,MGD,NAG,RMSprop,ADAM,Adadelta},  
x tick label style={rotate=45,anchor=east, font=\small}
]
\addplot 
	coordinates {(GD,22) (MGD,19)(NAG,18) (RMSprop,22) (ADAM,19) (Adadelta,22 )};
\addplot 
	coordinates {(GD,23) (MGD,22)(NAG,24) (RMSprop,23) (ADAM,23)(Adadelta,24)};
\addplot 
	coordinates {(GD,23) (MGD,23)(NAG,24) (RMSprop,23) (ADAM,23)(Adadelta,24)};
% \legend{T,P,TDA}
\end{axis}
\end{tikzpicture}
   \end{subfigure}
\begin{subfigure}{0.28 \textwidth}
 \caption{WGF}
\begin{tikzpicture}
\tikzstyle{every node}=[font=\small]
\begin{axis}[
	x tick label style={/pgf/number format/1000 sep=},
	height=5cm,
    width=\textwidth,
	ylabel=PSNR,
	enlargelimits=0.1,
	legend style={at={(0.5,1.1)},
	anchor=center,legend columns=-1},
	ybar,
	bar width = .1 cm,
	%ybar interval=0.7,
	symbolic x coords={GD,MGD,NAG,RMSprop,ADAM,Adadelta}, % these are the specification of coordinates on the x-axis. 
	xtick={GD,MGD,NAG,RMSprop,ADAM,Adadelta},  
x tick label style={rotate=45,anchor=east, font=\small}
]
\addplot 
	coordinates {(GD,44) (MGD,46)(NAG,47) (RMSprop,43) (ADAM,38) (Adadelta,44 )};
\addplot 
	coordinates {(GD,36) (MGD,36)(NAG,37) (RMSprop,34) (ADAM,32)(Adadelta,36)};
\addplot 
	coordinates {(GD,34) (MGD,36)(NAG,37) (RMSprop,34) (ADAM,32)(Adadelta,36)};
%\legend{T,P,TDA}
\end{axis}
\end{tikzpicture}
   
\end{subfigure}
\begin{subfigure}{0.28 \textwidth}
 \caption{Motion Blur}
\begin{tikzpicture}
\tikzstyle{every node}=[font=\small]
\begin{axis}[
	x tick label style={/pgf/number format/1000 sep=},
	height=5cm,
    width=\textwidth,
    ymin=-5, ymax=30,
	ylabel=PSNR,
	enlargelimits=0.1,
	legend style={at={(0.5,1.1)},
	anchor=center,legend columns=-1},
	ybar,
	bar width = .1 cm,
	%ybar interval=0.7,
	symbolic x coords={GD,MGD,NAG,RMSprop,ADAM,Adadelta}, % these are the specification of coordinates on the x-axis. 
	xtick={GD,MGD,NAG,RMSprop,ADAM,Adadelta},  
x tick label style={rotate=45,anchor=east, font=\small}
]
\addplot 
	coordinates {(GD,-52) (MGD,-146)(NAG,-176) (RMSprop,4) (ADAM,-19) (Adadelta,-40)};
\addplot 
	coordinates {(GD,24) (MGD,28)(NAG,27) (RMSprop,25) (ADAM,26)(Adadelta,24)};
\addplot 
	coordinates {(GD,23) (MGD,27)(NAG,27) (RMSprop,24) (ADAM,26)(Adadelta,23)};
%\legend{T,P,TDA}
\end{axis}
\end{tikzpicture}
   
\end{subfigure}
\begin{subfigure}{0.28 \textwidth}
 \caption{L0}
\begin{tikzpicture}
\tikzstyle{every node}=[font=\small]
\begin{axis}[
	x tick label style={/pgf/number format/1000 sep=},
	height=5cm,
    width=\textwidth,
	ylabel=PSNR,
	enlargelimits=0.1,
	legend style={at={(0.5,1.1)},
	anchor=center,legend columns=-1},
	ybar,
	bar width = .1 cm,
	%ybar interval=0.7,
	symbolic x coords={GD,MGD,NAG,RMSprop,ADAM,Adadelta}, % these are the specification of coordinates on the x-axis. 
	xtick={GD,MGD,NAG,RMSprop,ADAM,Adadelta},  
x tick label style={rotate=45,anchor=east, font=\small}
]
\addplot 
	coordinates {(GD,27) (MGD,22)(NAG,22) (RMSprop,28) (ADAM,23) (Adadelta,27)};
\addplot 
	coordinates {(GD,27) (MGD,22)(NAG,24) (RMSprop,27) (ADAM,23)(Adadelta,26)};
\addplot 
	coordinates {(GD,25) (MGD,19)(NAG,20) (RMSprop,27) (ADAM,22)(Adadelta,27)};
%\legend{T,P,TDA}
\end{axis}
\end{tikzpicture}
   
\end{subfigure}
\begin{subfigure}{0.28 \textwidth}
 \caption{RTV}
\begin{tikzpicture}
\tikzstyle{every node}=[font=\small]
\begin{axis}[
	x tick label style={/pgf/number format/1000 sep=},
	height=5cm,
    width=\textwidth,
	ylabel=PSNR,
	enlargelimits=0.1,
	legend style={at={(0.5,1.1)},
	anchor=center,legend columns=-1},
	ybar,
	bar width = .1 cm,
	%ybar interval=0.7,
	symbolic x coords={GD,MGD,NAG,RMSprop,ADAM,Adadelta}, % these are the specification of coordinates on the x-axis. 
	xtick={GD,MGD,NAG,RMSprop,ADAM,Adadelta},  
x tick label style={rotate=45,anchor=east, font=\small}
]
\addplot 
	coordinates {(GD,31) (MGD,29)(NAG,31) (RMSprop,31) (ADAM,29) (Adadelta,31)};
\addplot 
	coordinates {(GD,28) (MGD,24)(NAG,27) (RMSprop,27) (ADAM,24)(Adadelta,28)};
\addplot 
	coordinates {(GD,27) (MGD,21)(NAG,22) (RMSprop,27) (ADAM,23)(Adadelta,28)};
%\legend{T,P,TDA}
\end{axis}
\end{tikzpicture}
   
\end{subfigure}
\begin{subfigure}{0.28 \textwidth}
 \caption{RGF}
\begin{tikzpicture}
\tikzstyle{every node}=[font=\small]
\begin{axis}[
	x tick label style={/pgf/number format/1000 sep=},
	height=5cm,
    width=\textwidth,
	ylabel=PSNR,
	enlargelimits=0.1,
	legend style={at={(0.5,1.1)},
	anchor=center,legend columns=-1},
	ybar,
	bar width = .1 cm,
	%ybar interval=0.7,
	symbolic x coords={GD,MGD,NAG,RMSprop,ADAM,Adadelta}, % these are the specification of coordinates on the x-axis. 
	xtick={GD,MGD,NAG,RMSprop,ADAM,Adadelta},  
x tick label style={rotate=45,anchor=east, font=\small}
]
\addplot 
	coordinates {(GD,10) (MGD,-9)(NAG,-6) (RMSprop,11) (ADAM,1) (Adadelta,11)};
\addplot 
	coordinates {(GD,24) (MGD,-1)(NAG,17) (RMSprop,24) (ADAM,13)(Adadelta,24)};
\addplot 
	coordinates {(GD,23) (MGD,-9)(NAG,0) (RMSprop,24) (ADAM,12)(Adadelta,24)};
%\legend{T,P,TDA}
\end{axis}
\end{tikzpicture}
   
\end{subfigure}
\begin{subfigure}{0.28 \textwidth}
 \caption{WLS}
\begin{tikzpicture}
\tikzstyle{every node}=[font=\small]
\begin{axis}[
	x tick label style={/pgf/number format/1000 sep=},
	height=5cm,
    width=\textwidth,
	ylabel=PSNR,
	enlargelimits=0.1,
	legend style={at={(0.5,-0.6)},
	anchor=center,legend columns=-1},
	ybar,
	bar width = .1 cm,
	%ybar interval=0.7,
	symbolic x coords={GD,MGD,NAG,RMSprop,ADAM,Adadelta}, % these are the specification of coordinates on the x-axis. 
	xtick={GD,MGD,NAG,RMSprop,ADAM,Adadelta},  
x tick label style={rotate=45,anchor=east, font=\small}
]
\addplot 
	coordinates {(GD,30) (MGD,26)(NAG,29) (RMSprop,29) (ADAM,28) (Adadelta,30)};
\addplot 
	coordinates {(GD,27) (MGD,23)(NAG,27) (RMSprop,27) (ADAM,26)(Adadelta,28)};
\addplot 
	coordinates {(GD,27) (MGD,23)(NAG,26) (RMSprop,27) (ADAM,26)(Adadelta,28)};
\legend{T,P,TDA}
\end{axis}
\end{tikzpicture}
   
\end{subfigure}
\begin{subfigure}{0.28 \textwidth}
 \caption{Disk Kernel}
\begin{tikzpicture}
\tikzstyle{every node}=[font=\small]
\begin{axis}[
	x tick label style={/pgf/number format/1000 sep=},
	height=5cm,
    width=\textwidth,
    ymin=-5, ymax=35,
	ylabel=PSNR,
	enlargelimits=0.1,
	legend style={at={(0.5,1.1)},
	anchor=center,legend columns=-1},
	ybar,
	bar width = .1 cm,
	%ybar interval=0.7,
	symbolic x coords={GD,MGD,NAG,RMSprop,ADAM,Adadelta}, % these are the specification of coordinates on the x-axis. 
	xtick={GD,MGD,NAG,RMSprop,ADAM,Adadelta},  
x tick label style={rotate=45,anchor=east, font=\small}
]
\addplot 
	coordinates {(GD,-14) (MGD,-90)(NAG,-106) (RMSprop,5) (ADAM,-18) (Adadelta,-10)};
\addplot 
	coordinates {(GD,27) (MGD,31)(NAG,31) (RMSprop,27) (ADAM,28)(Adadelta,28)};
\addplot 
	coordinates {(GD,26) (MGD,30)(NAG,30) (RMSprop,27) (ADAM,28)(Adadelta,27)};
%\legend{T,P,TDA}
\end{axis}
\end{tikzpicture}
   
\end{subfigure}

\caption{nkhjh }
\label{fig:reversingGFcomparison}
\end{figure*}

==> accGradientDescent.tex <==
% \newpage

\subsection{Performance improvement by using accelerated gradient descent methods}

Accelerated gradient descent (AGD) methods \cite{optimizationAlgo} such as Momemtum, Nesterov, RMSprop, Adam and adadelta were developed to tackle problems related gradient descend. For example, when the gradient is consistently small the convergence is very slow since $\boldsymbol{x}$ only updates its value based on the gradient at each iteration only. In addition, noisy gradients can make gradient descent to follow the wrong direction and end up in a local minimum. AGD methods are widely used  training deep neural networks and have the potential to reduce the number of iterations needed to achieve convergence and to increase the robustness against noisy gradients. 

Since both the P-method and the proposed TDA-method can be interpreted as gradient descent algorithms using different approximation of the gradient, it is a natural to apply the many well known AGD methods to test if they can improve the performance of these two algorithms. For easy reference, in the Appendix we present a brief summary of AGD methods studied in this work. We test above the AGS methods on the proposed TDA-method and the P-method. The tests are conducted by replacing the gradient of each method by the following approximations. 

\begin{itemize}
    \item TDA-method: $\nabla f(\boldsymbol{x_{k}})=g(\boldsymbol{x}_{k}+\boldsymbol{h}_{k})-g(\boldsymbol{x}_{k})$
    % \item T-method: $\nabla f(\boldsymbol{x_{k}})=h_{k}$
    \item P-method: $\nabla f(\boldsymbol{x_{k}}) = \frac{||\boldsymbol{h}_{k}||}{||g(\boldsymbol{x}_{k}+\boldsymbol{h}_{k})-g(\boldsymbol{x}_{k}-\boldsymbol{h}_{k})||} (g(\boldsymbol{x}_{k}+\boldsymbol{h}_{k})-g(\boldsymbol{x}_{k}-\boldsymbol{h}_{k}))$
\end{itemize}
Here for consistence of notation, we have used bold face fonts $\boldsymbol{x}_k$ and $\boldsymbol{h}_k$ for the tow image variables.  We present the test results in section \ref{sec:AGD results}. 
%We define here some of the methods to accelerate the convergence of GD algorithm. Recalling gradient descent (Eq.\ref{eq:GD}), the variable to be optimized is updated at every iteration based on the gradients, gradually approximating to an optimal value where gradients are zero. 
%
%\begin{equation}
%\boldsymbol{x}_{k+1}=\boldsymbol{x}_{k}-\lambda\na%bla J(\boldsymbol{x}_{k})
%\label{eq:GD}
%\end{equation}

%The step size $\lambda$ controls the contribution of each iteration to the result, typically $ \lambda \in (0, 1]$. Ass discussed earlier, in our method the gradient $\nabla J(\boldsymbol{x}_{k})$ is replaced by the forward difference $g(x_{k}+h_{k})-g(x_{k})$. 

% The so called T and P method approximate $\nabla J(\boldsymbol{x}_{k})$ differently but the final algorithm can be reduced as gradient descent as well, so we follow the intuition that AGD techniques could be employed to improve other reverse filter methods.





==> table2.tex <==
\begin{table}[]
\centering
\caption{Optimization methods. }
\label{tab:agd_table}
\renewcommand{\arraystretch}{2}
\begin{tabular}{lll}
                                        &                                                                                                                                  &                                                                                                                                                                                                                                                                                                                                                                                                \\ \cline{2-3} 
\multicolumn{1}{l|}{}                   & \multicolumn{1}{l|}{\textbf{$\Delta x_k$}}                                                                                       & \multicolumn{1}{l|}{}                                                                                                                                                                                                                                                                                                                                                                          \\ \hline
\multicolumn{1}{|l|}{\textbf{GD}}       & \multicolumn{1}{l|}{$ \lambda\nabla J(\boldsymbol{x}_{k})$}                                                                      & \multicolumn{1}{l|}{}                                                                                                                                                                                                                                                                                                                                                                          \\ \hline
\multicolumn{1}{|l|}{\textbf{MGD}}      & \multicolumn{1}{l|}{$  \lambda \nabla f(\boldsymbol{x}_k) + \beta \boldsymbol{v}_{k-1}$}                                         & \multicolumn{1}{l|}{}                                                                                                                                                                                                                                                                                                                                                                          \\ \hline
\multicolumn{1}{|l|}{\textbf{NAG}}      & \multicolumn{1}{l|}{$ \lambda \nabla f(\hat{\boldsymbol{x}}_k) + \beta \boldsymbol{v}_{k-1} $}                                   & \multicolumn{1}{l|}{$ \hat{\boldsymbol{x}}_{k} = x_k + \beta v_{k-1} $}                                                                                                                                                                                                                                                                                                                        \\ \hline
\multicolumn{1}{|l|}{\textbf{Adagrad}}  & \multicolumn{1}{l|}{$  \frac{\lambda}{\sqrt{v_{k}+\epsilon}} \nabla f(\boldsymbol{x}_k) $}                                       & \multicolumn{1}{l|}{$ \boldsymbol{v}_{k} = \boldsymbol{v}_{k-1} + \beta \nabla f(\boldsymbol{x}_k)^2$}                                                                                                                                                                                                                                                                                         \\ \hline
\multicolumn{1}{|l|}{\textbf{RMSprop}}  & \multicolumn{1}{l|}{$ \frac{\lambda}{\sqrt{\boldsymbol{v}_k+\epsilon}}\nabla f(\boldsymbol{x}_k)$}                               & \multicolumn{1}{l|}{$ \boldsymbol{v}_k = \beta \boldsymbol{v}_{k-1} +(1- \beta)\nabla f(\boldsymbol{x}_k)^2$}                                                                                                                                                                                                                                                                                  \\ \hline
\multicolumn{1}{|l|}{\textbf{Adadelta}} & \multicolumn{1}{l|}{$\frac{\sqrt{\boldsymbol{u}_{k-1}+\epsilon}}{\sqrt{\boldsymbol{v}_{k}+\epsilon}}\nabla f(\boldsymbol{x}_k)$} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}$ \boldsymbol{u}_{k} = \beta \boldsymbol{u}_{k-1}  + (1-\beta) \Delta \boldsymbol{x}_{k}^2$\\ $ \boldsymbol{v}_{k} = \beta \boldsymbol{v}_{k-1}  + (1-\beta) \nabla f(\boldsymbol{x}_k)^2$\end{tabular}}                                                                                                                                        \\ \hline
\multicolumn{1}{|l|}{\textbf{Adam}}     & \multicolumn{1}{l|}{$\lambda \frac{\boldsymbol{\hat{m}_k}}{\sqrt{\boldsymbol{\hat{v}_k}}+\epsilon}$}                             & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}$ \boldsymbol{m_k} = \beta_1 \boldsymbol{m_{k-1}} + (1-\beta_1) \nabla f(\boldsymbol{x}_k) $\\ $ \boldsymbol{v_k} = \beta_2 \boldsymbol{v_{k-1}} + (1-\beta_2) \nabla f(\boldsymbol{x}_k)^2 $\\ $  \boldsymbol{\hat{m}_k} = \frac{\boldsymbol{m_k} }{1-\beta_1}$\\ $ \boldsymbol{\hat{v}_k}= \frac{ \boldsymbol{v_k}}{1-\beta_2}$\end{tabular}} \\ \hline
\end{tabular}
\end{table}
